Report of the Snowmass 2013 energy frontier QCD working group

This is the summary report of the energy frontier QCD working group prepared for Snowmass 2013. We review the status of tools, both theoretical and experimental, for understanding the strong interactions at colliders. We attempt to prioritize important directions that future developments should take. Most of the efforts of the QCD working group concentrate on proton-proton colliders, at 14 TeV as planned for the next run of the LHC, and for 33 and 100 TeV, possible energies of the colliders that will be necessary to carry on the physics program started at 14 TeV. We also examine QCD predictions and measurements at lepton-lepton and lepton-hadron colliders, and in particular their ability to improve our knowledge of strong coupling constant and parton distribution functions.

==> QCD/TotCS-Mll-cuts_ZNul_LHC100_mstw.dat.tex <==
 % Total cs for different cuts at the LHC       
 %************************************************
 % PDFs : mstw
 % M_{\ell\ell}^{\mathrm{min}}/(\GeV)            &                100.0 &                200.0 &                400.0 &               1000.0 &               2000.0 &               4000.0 \\ 
%-------------------------------------------------
   $$ \begin{array}{c|rrrrrr} 
 \multicolumn{7}{c}{\Pp\Pp
                                                                    \to l^+l^-\; \mathrm{jet} + X \;\mbox{at} \;\sqrt{s} =100 \TeV} \\
              \hline M_{ll} / \GeV & 100-\infty \;\;\; & 200-\infty \;\;\; & 400-\infty \;\; & 1000-\infty \;\; & 2000-\infty \;\; & 4000-\infty \; \\ 
  \hline \hline 
                 \si_{\born}^{\mu = \MZ}/\pba \; & \;               60.70(2)                  \; & \;              5.3194(9)                  \; & \;              0.9142(1)                  \; & \;             0.08462(1)                  \; & \;            0.012762(2)                  \; & \;           0.0016229(2)                  \\ 
              \si_{\born}^{\mathrm{var}}/\pba \; & \;               61.76(2)                  \; & \;              5.3548(9)                  \; & \;              0.9016(1)                  \; & \;             0.07980(1)                  \; & \;            0.011500(2)                  \; & \;           0.0013850(2)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                   \de_{\EW}^{\mu = \MZ} / \% \; & \;                -9.4(1)                  \; & \;               -5.85(1)                  \; & \;               -8.41(1)                  \; & \;              -14.28(2)                  \; & \;              -21.05(3)                  \; & \;              -29.97(5)                  \\ 
    \de_{\EW}^{\mathrm{rec}\,,\mu = \MZ} / \% \; & \;                -5.0(1)                  \; & \;               -3.23(1)                  \; & \;               -5.29(1)                  \; & \;              -10.42(3)                  \; & \;              -16.42(3)                  \; & \;              -24.34(5)                  \\ 
 %--------------------------------------------------
 \hline 
                  \de_{\EW}^{\mathrm{var}}/\% \; & \;                -9.5(2)                  \; & \;               -5.76(1)                  \; & \;               -8.31(1)                  \; & \;              -14.08(2)                  \; & \;              -20.85(3)                  \; & \;              -29.87(5)                  \\ 
   \de_{\EW}^{\mathrm{rec}\,,\mathrm{var}}/\% \; & \;                -5.2(2)                  \; & \;               -3.07(1)                  \; & \;               -5.15(2)                  \; & \;              -10.11(2)                  \; & \;              -16.22(4)                  \; & \;              -24.09(5)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                    \de_{\QCD}^{\mu = \MZ}/\% \; & \;                 36.(4)                  \; & \;                20.8(3)                  \; & \;                 7.3(2)                  \; & \;               -18.1(1)                  \; & \;               -43.3(1)                  \; & \;               -73.7(1)                  \\ 
                 \de_{\QCD}^{\mathrm{var}}/\% \; & \;                29.3(9)                  \; & \;                18.4(3)                  \; & \;                 6.0(1)                  \; & \;               -16.3(1)                  \; & \;               -37.4(1)                  \; & \;               -63.3(1)                  \\ 
 %--------------------------------------------------
 \hline 
              \de_{\QCD,\veto}^{\mu = \MZ}/\% \; & \;                 5.0(9)                  \; & \;                -7.0(2)                  \; & \;               -21.2(2)                  \; & \;               -46.8(1)                  \; & \;               -71.8(1)                  \; & \;              -102.1(1)                  \\ 
           \de_{\QCD,\veto}^{\mathrm{var}}/\% \; & \;                 3.8(7)                  \; & \;                -7.4(3)                  \; & \;               -19.6(2)                  \; & \;               -41.7(1)                  \; & \;               -63.1(1)                  \; & \;               -88.5(2)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
               \de_{\ga,\born}^{\mu = \MZ}/\% \; & \;               0.532(1)                  \; & \;               1.679(4)                  \; & \;               2.019(6)                  \; & \;               1.988(6)                  \; & \;               1.792(6)                  \; & \;               1.511(4)                  \\ 
            \de_{\ga,\born}^{\mathrm{var}}/\% \; & \;               0.568(1)                  \; & \;               1.871(4)                  \; & \;               2.363(7)                  \; & \;               2.464(7)                  \; & \;               2.259(7)                  \; & \;               1.901(5)                  \\ 
 %--------------------------------------------------
 \hline \hline
 %                \de_{\ga,\NLO}^{\mu = \MZ}/\% \; & \;               0.532(1)                  \; & \;               1.679(4)                  \; & \;               2.019(6)                  \; & \;               1.988(6)                  \; & \;               1.792(6)                  \; & \;               1.511(4)                  \\ 
 %             \de_{\ga,\NLO}^{\mathrm{var}}/\% \; & \;               0.568(1)                  \; & \;               1.871(4)                  \; & \;               2.363(7)                  \; & \;               2.464(7)                  \; & \;               2.259(7)                  \; & \;               1.901(5)                  \\ 
 % %--------------------------------------------------
 % \hline 
 %          \de_{\ga,\NLO,\veto}^{\mu = \MZ}/\% \; & \;               0.532(1)                  \; & \;               1.679(4)                  \; & \;               2.019(6)                  \; & \;               1.988(6)                  \; & \;               1.792(6)                  \; & \;               1.511(4)                  \\ 
 %       \de_{\ga,\NLO,\veto}^{\mathrm{var}}/\% \; & \;               0.568(1)                  \; & \;               1.871(4)                  \; & \;               2.363(7)                  \; & \;               2.464(7)                  \; & \;               2.259(7)                  \; & \;               1.901(5)                  \\ 
 % %--------------------------------------------------
 % %--------------------------------------------------
 %  \hline \hline 
 %                    \de_{\Int}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %                 \de_{\Int}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 % %--------------------------------------------------
 % \hline 
 %              \de_{\Int,\veto}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %           \de_{\Int,\veto}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 % %--------------------------------------------------
 % %--------------------------------------------------
     \si_{\full,\veto}^{\mathrm{var}}/\pba/\% \; & \;                58.6(4)                  \; & \;                4.75(1)                  \; & \;               0.672(1)                  \; & \;              0.0373(1)                  \; & \;             0.00211(2)                  \; & \;           -0.000228(3)                  \\ 
\end{array}$$


==> QCD/TotCS-Mll-cuts_ZNul_LHC33_mstw.dat.tex <==
% Total cs for different cuts at the LHC       
%************************************************
% PDFs : mstw
% M_{\ell\ell}^{\mathrm{min}}/(\GeV)            &                100.0 &                200.0 &                400.0 &               1000.0 &               2000.0 &               4000.0 \\ 
%-------------------------------------------------
%%                                                              $$ 
$$
\begin{array}{c|rrrrrr}
                                                                  \multicolumn{7}{c}{\Pp\Pp
                                                                    \to l^+l^-\; \mathrm{jet} + X \;\mbox{at} \;\sqrt{s} =33 \TeV} \\
              \hline M_{ll} / \GeV & 100-\infty \;\;\; & 200-\infty \;\;\; & 400-\infty \;\; & 1000-\infty \;\; & 2000-\infty \;\; & 4000-\infty \; \\  
 \hline \hline 
                 \si_{\born}^{\mu = \MZ}/\pba \; & \;              19.924(6)                  \; & \;              1.6890(2)                  \; & \;             0.28005(4)                  \; & \;            0.022682(3)                  \; & \;           0.0024968(4)                  \; & \;          0.00015626(2)                  \\ 
              \si_{\born}^{\mathrm{var}}/\pba \; & \;              19.849(6)                  \; & \;              1.6482(2)                  \; & \;             0.26618(4)                  \; & \;            0.020604(3)                  \; & \;           0.0021755(3)                  \; & \;          0.00012945(2)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                   \de_{\EW}^{\mu = \MZ} / \% \; & \;                -9.6(1)                  \; & \;               -5.74(1)                  \; & \;               -8.26(1)                  \; & \;              -14.31(2)                  \; & \;              -21.69(3)                  \; & \;              -31.92(4)                  \\ 
    \de_{\EW}^{\mathrm{rec}\,,\mu = \MZ} / \% \; & \;                -5.3(1)                  \; & \;               -3.06(1)                  \; & \;               -5.13(1)                  \; & \;              -10.11(2)                  \; & \;              -16.34(3)                  \; & \;              -24.77(4)                  \\ 
 %--------------------------------------------------
 \hline 
                  \de_{\EW}^{\mathrm{var}}/\% \; & \;               -9.46(8)                  \; & \;               -5.69(1)                  \; & \;               -8.14(1)                  \; & \;              -14.18(2)                  \; & \;              -21.56(3)                  \; & \;              -31.88(6)                  \\ 
   \de_{\EW}^{\mathrm{rec}\,,\mathrm{var}}/\% \; & \;               -5.05(7)                  \; & \;               -2.94(1)                  \; & \;               -4.93(1)                  \; & \;               -9.93(2)                  \; & \;              -16.14(3)                  \; & \;              -24.75(6)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                    \de_{\QCD}^{\mu = \MZ}/\% \; & \;                 29.(1)                  \; & \;                14.8(2)                  \; & \;                -0.6(1)                  \; & \;               -29.5(1)                  \; & \;               -57.1(1)                  \; & \;               -89.5(1)                  \\ 
                 \de_{\QCD}^{\mathrm{var}}/\% \; & \;                27.9(6)                  \; & \;                15.9(2)                  \; & \;                 2.2(1)                  \; & \;               -23.0(1)                  \; & \;               -46.6(1)                  \; & \;               -74.8(1)                  \\ 
 %--------------------------------------------------
 \hline 
              \de_{\QCD,\veto}^{\mu = \MZ}/\% \; & \;                 5.0(6)                  \; & \;                -8.9(2)                  \; & \;               -25.5(1)                  \; & \;               -54.9(1)                  \; & \;               -82.4(1)                  \; & \;              -115.3(1)                  \\ 
           \de_{\QCD,\veto}^{\mathrm{var}}/\% \; & \;                 6.1(4)                  \; & \;                -7.2(2)                  \; & \;               -20.8(2)                  \; & \;               -45.8(1)                  \; & \;               -69.8(1)                  \; & \;               -98.1(1)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
               \de_{\ga,\born}^{\mu = \MZ}/\% \; & \;               0.669(1)                  \; & \;               2.097(5)                  \; & \;               2.409(6)                  \; & \;               2.168(6)                  \; & \;               1.844(5)                  \; & \;               1.610(3)                  \\ 
            \de_{\ga,\born}^{\mathrm{var}}/\% \; & \;               0.710(1)                  \; & \;               2.298(5)                  \; & \;               2.721(7)                  \; & \;               2.510(7)                  \; & \;               2.135(5)                  \; & \;               1.822(3)                  \\ 
 %--------------------------------------------------
 \hline \hline
 %                \de_{\ga,\NLO}^{\mu = \MZ}/\% \; & \;               0.669(1)                  \; & \;               2.097(5)                  \; & \;               2.409(6)                  \; & \;               2.168(6)                  \; & \;               1.844(5)                  \; & \;               1.610(3)                  \\ 
 %             \de_{\ga,\NLO}^{\mathrm{var}}/\% \; & \;               0.710(1)                  \; & \;               2.298(5)                  \; & \;               2.721(7)                  \; & \;               2.510(7)                  \; & \;               2.135(5)                  \; & \;               1.822(3)                  \\ 
 % %--------------------------------------------------
 % \hline 
 %          \de_{\ga,\NLO,\veto}^{\mu = \MZ}/\% \; & \;               0.669(1)                  \; & \;               2.097(5)                  \; & \;               2.409(6)                  \; & \;               2.168(6)                  \; & \;               1.844(5)                  \; & \;               1.610(3)                  \\ 
 %       \de_{\ga,\NLO,\veto}^{\mathrm{var}}/\% \; & \;               0.710(1)                  \; & \;               2.298(5)                  \; & \;               2.721(7)                  \; & \;               2.510(7)                  \; & \;               2.135(5)                  \; & \;               1.822(3)                  \\ 
 % %--------------------------------------------------
 % %--------------------------------------------------
 %  \hline \hline 
 %                    \de_{\Int}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %                 \de_{\Int}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 % %--------------------------------------------------
 % \hline 
 %              \de_{\Int,\veto}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %           \de_{\Int,\veto}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 % %--------------------------------------------------
 % %--------------------------------------------------
     \si_{\full,\veto}^{\mathrm{var}}/\pba/\% \; & \;               19.32(9)                  \; & \;               1.473(4)                  \; & \;              0.1965(6)                  \; & \;             0.00877(2)                  \; & \;            0.000234(3)                  \; & \;          -0.0000365(2)                  \\ 
\end{array}
$$


==> QCD/TotCS-ptj-cuts_ZNul_LHC33_mstw.dat.tex <==
                                                                                                                                       $$ \begin{array}{c|rrrrrr}
                                                                  \multicolumn{7}{c}{\Pp\Pp
                                                                    \to l^+l^-\; \mathrm{jet} + X \;\mbox{at} \;\sqrt{s} =33 \TeV} \\
              \hline p_{\rT,\mathrm{jet}} / \GeV & 50-\infty \;\;\; & 100-\infty \;\;\; & 200-\infty \;\; & 400-\infty \;\; & 1000-\infty \;\; & 2000-\infty \; \\ 
  \hline \hline 
                 \si_{\born}^{\mu = \MZ}/\pba \; & \;              121.26(1)                  \; & \;              33.737(4)                  \; & \;              6.3314(7)                  \; & \;             0.79429(9)                  \; & \;            0.026920(2)                  \; & \;           0.0010264(1)                  \\ 
              \si_{\born}^{\mathrm{var}}/\pba \; & \;              120.70(1)                  \; & \;              32.654(4)                  \; & \;              5.6403(7)                  \; & \;             0.60157(6)                  \; & \;            0.014491(1)                  \; & \;          0.00038663(4)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                   \de_{\EW}^{\mu = \MZ} / \% \; & \;               -4.68(1)                  \; & \;               -5.47(1)                  \; & \;               -9.25(1)                  \; & \;              -16.15(2)                  \; & \;              -29.25(5)                  \; & \;               -41.8(2)                  \\ 
    \de_{\EW}^{\mathrm{rec}\,,\mu = \MZ} / \% \; & \;               -3.29(3)                  \; & \;               -4.48(2)                  \; & \;               -8.50(4)                  \; & \;              -15.42(3)                  \; & \;              -28.59(8)                  \; & \;               -41.0(1)                  \\ 
 %--------------------------------------------------
 \hline 
                  \de_{\EW}^{\mathrm{var}}/\% \; & \;               -4.61(1)                  \; & \;               -5.31(1)                  \; & \;               -8.92(1)                  \; & \;              -15.65(2)                  \; & \;              -28.48(5)                  \; & \;               -40.5(3)                  \\ 
   \de_{\EW}^{\mathrm{rec}\,,\mathrm{var}}/\% \; & \;               -3.16(3)                  \; & \;               -4.42(4)                  \; & \;               -8.12(2)                  \; & \;              -14.89(2)                  \; & \;              -27.62(5)                  \; & \;               -39.9(1)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
                    \de_{\QCD}^{\mu = \MZ}/\% \; & \;                56.1(2)                  \; & \;                78.7(1)                  \; & \;               113.0(1)                  \; & \;               160.5(1)                  \; & \;               240.4(2)                  \; & \;               330.6(3)                  \\ 
                 \de_{\QCD}^{\mathrm{var}}/\% \; & \;                54.0(1)                  \; & \;                77.4(1)                  \; & \;               117.3(1)                  \; & \;               186.0(1)                  \; & \;               347.2(2)                  \; & \;               609.0(4)                  \\ 
 %--------------------------------------------------
 \hline 
              \de_{\QCD,\veto}^{\mu = \MZ}/\% \; & \;                13.1(1)                  \; & \;                23.3(1)                  \; & \;                29.7(1)                  \; & \;                27.5(1)                  \; & \;                -2.8(1)                  \; & \;               -42.2(1)                  \\ 
           \de_{\QCD,\veto}^{\mathrm{var}}/\% \; & \;                12.9(1)                  \; & \;                25.6(2)                  \; & \;                38.8(1)                  \; & \;                49.8(1)                  \; & \;                52.6(1)                  \; & \;                54.0(1)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
  \hline \hline 
               \de_{\ga,\born}^{\mu = \MZ}/\% \; & \;              0.1377(4)                  \; & \;              0.1647(4)                  \; & \;              0.1960(5)                  \; & \;              0.2442(7)                  \; & \;               0.341(1)                  \; & \;               0.457(1)                  \\ 
            \de_{\ga,\born}^{\mathrm{var}}/\% \; & \;              0.1489(4)                  \; & \;              0.1923(5)                  \; & \;              0.2562(7)                  \; & \;               0.371(1)                  \; & \;               0.661(2)                  \; & \;               1.095(3)                  \\ 
 %--------------------------------------------------
 \hline\hline 
%                \de_{\ga,\NLO}^{\mu = \MZ}/\% \; & \;              0.1377(4)                  \; & \;              0.1647(4)                  \; & \;              0.1960(5)                  \; & \;              0.2442(7)                  \; & \;               0.341(1)                  \; & \;               0.457(1)                  \\ 
%             \de_{\ga,\NLO}^{\mathrm{var}}/\% \; & \;              0.1489(4)                  \; & \;              0.1923(5)                  \; & \;              0.2562(7)                  \; & \;               0.371(1)                  \; & \;               0.661(2)                  \; & \;               1.095(3)                  \\ 
 %--------------------------------------------------
% \hline 
%          \de_{\ga,\NLO,\veto}^{\mu = \MZ}/\% \; & \;              0.1377(4)                  \; & \;              0.1647(4)                  \; & \;              0.1960(5)                  \; & \;              0.2442(7)                  \; & \;               0.341(1)                  \; & \;               0.457(1)                  \\ 
%       \de_{\ga,\NLO,\veto}^{\mathrm{var}}/\% \; & \;              0.1489(4)                  \; & \;              0.1923(5)                  \; & \;              0.2562(7)                  \; & \;               0.371(1)                  \; & \;               0.661(2)                  \; & \;               1.095(3)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
%  \hline \hline 
%                    \de_{\Int}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
%                 \de_{\Int}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %--------------------------------------------------
% \hline 
%              \de_{\Int,\veto}^{\mu = \MZ}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
%           \de_{\Int,\veto}^{\mathrm{var}}/\% \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \; & \;              0.0000(0)                  \\ 
 %--------------------------------------------------
 %--------------------------------------------------
     \si_{\full,\veto}^{\mathrm{var}}/\pba/\% \; & \;               130.9(2)                  \; & \;               39.36(6)                  \; & \;               7.342(9)                  \; & \;              0.8091(7)                  \; & \;             0.01808(2)                  \; & \;            0.000443(1)                  \\ 
 \end{array} $$

==> QCD/qcd-JetETmiss-Pileup-ATLAS.tex <==

Both the precision and the discovery physics programs at the 14 TeV LHC and at future colliders require
high instantaneous luminosities. This will result in the presence of a large number of additional
interactions for every crossing, and the subsequent difficulties in triggering on interesting physics
and then in removing the effects of the pileup to recover the original physics. Pileup is one of the
main challenges for jets and missing transverse energy, with both the presence of additional energy
(offset) as well as the creation of additional fake jets due to local fluctuations in the energy
density.   Thus, it is important to develop the tools needed for removing the effects of pileup in
order to insure that precise measurements can still be undertaken at high luminosities. 

A study was carried out within the ATLAS full simulation framework, using topological clustering and
local hadron calibration, where samples with up to 200 pileup events per crossing (with both $50$ns and
$25$ns bunch structure) were used. 
Topoclusters are an attempt to reconstruct three-dimensional energy deposits in the calorimeter and are
built using a nearest-neighbor algorithm that clusters calorimeter cells with energy significance
($|E_{cell}|/\sigma$)~$>4$~for the seed, $>2$~for neighbors, and $>0$~at the boundary. $E_{cell}$ is
calibrated using information derived from test beam and detailed GEANT4 simulations (EM scale) and
$\sigma$ is the sum in quadrature of the electronic and expected pileup noise, as described in
Sec. 10.5.2 of Ref.~\cite{Aad:2008zzm}. Topoclusters can be further calibrated using local
information (LCW) as described in Ref.~\cite{Cojocaru:2004jk}.  

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.4\linewidth]{QCD/rhoLCDist_25ns_approved.pdf}
\includegraphics[width=0.4\linewidth]{QCD/rhoLCVsMu_25ns_approved-eps-converted-to.pdf}
\end{center}
\caption{Distributions of the event-by-event median $p_{T}$ density ($\rho$) for different values of the mean number of interactions per bunch crossing
$\langle\mu\rangle$ (left) and the dependence of $\rho$ on the mean number of interactions per bunch crossing (right).}
\label{fig:rho}
\end{figure}
Figure~\ref{fig:rho} shows an example of an  event where hard jets are embedded in a background of soft
energy resulting from multiple minimum bias events. An effective density $\rho$ can be determined on an
event-by-event basis~\cite{Cacciari:2007fd} based on energy depositions outside hard jets.  The
corrected jet transverse momentum can be calculated by subtracting the contribution due to pileup
$\rho A^{jet}$, where $A^{jet}$ is the active area of the jet. The technique works since the pileup density depends
linearly on the number of interactions up to very high values of the average number of pileup events.
As can be seen in Fig.~\ref{fig:rho}, the optimization of $\sigma$ pileup noise during topocluster formation is
critical to suppress pileup contributions at high luminosity. When the pileup noise used in
topoclustering is chosen to match the pileup conditions, a significant reduction on the event $p_T$
density is achieved. 
Although the event-by-event pileup subtraction accounts for global pileup fluctuations from one event to
another, it is not sensitive to local fluctuations. A residual correction is necessary to account for
the higher occupancy inside jets and for out-of-time pileup effects. 

The jet calibration scheme has been shown to work well up to very high luminosities. The pileup
subtraction technique restores the jet energy response to that of jets in the presence of no pileup. 
The pileup subtraction also significantly reduces the number of fake (pileup) events per jet, as shown
in Fig.~\ref{fig:fakes}. There are approximately $3$ ($0.5$) pileup jets with $p_T> 20$ ($40$) GeV per event,
with approximately $140$ additional interactions per crossing. Further improvements can be expected using
tracking and vertexing information. 
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.5\linewidth]{QCD/PUJetMultiplicity_BeforAndAfter_JetArea_symmetricMu140_newlegend_approved.pdf}
\end{center}
\caption{The mean pileup jet multiplicity as a function of the number of truth vertices $N_{vtx}$ in events with an average number
of interactions per bunch crossing, $\langle\mu\rangle=140$. A pileup-jet is defined as a reconstructed jet that is not closely matched in $\Delta R$ to a truth jet.}
\label{fig:fakes}
\end{figure}


The jet energy resolution at low jet transverse momentum degrades in the presence of pileup; there are
local pileup fluctuations within events, not captured by the global event-by-event energy density used
in the calibration. The result is an effective noise term whose magnitude increases as the square root
of the average number of additional interactions. A reduction of local pileup fluctuations may be
possible using tracking information and advanced subtraction techniques using more local information.
Figure~\ref{fig:resolution} shows the dependence of the fractional jet energy resolution and the noise term
on an average number of interactions per bunch crossing, $\langle\mu\rangle$. The square root dependence of the noise term indicates that the degradation in
resolution is due to pileup fluctuations and there are no additional contributions from no-linear
effects of topoclustering or local hadron calibration. 
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.45\linewidth]{QCD/muScan3_Sym_25nsresolutionVsPtKt4EMTopo_approved.pdf}
\includegraphics[width=0.415\linewidth]{QCD/NoiseVsMu_Sym_25ns_0_approved.pdf}
\end{center}
\caption{The fractional jet energy resolution as a function of jet $p_{T}$ for different values of the mean number of interactions
per bunch crossing (left) and the noise term of the jet energy resolution as a function of $\langle\mu\rangle$ (right).}
\label{fig:resolution}
\end{figure}


Jet substructure is a key technique for the reconstruction of boosted objects. Grooming algorithms
significantly reduce the sensitivity to pileup, due to the reduced jet area. The original jet mass can
be recovered, with reasonably low degradation of mass resolution. Figure~\ref{fig:boost} shows the jet
mass distribution in $Z^{\prime} \rightarrow t \bar{t}$ events before and after the application of trimming,
for increasing values of $\langle\mu\rangle$. Trimming is implemented by re-clustering the jet into subjets of
radius $R=0.3$. The clusters belonging to subjets that carry at least $5\%$ of the original jet $p_T$ are
kept, and those clusters in subjets with less than $5\%$ of the original jet $p_T$ are discarded.
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.4\linewidth]{QCD/boost1.pdf}
\includegraphics[width=0.4\linewidth]{QCD/boost2.pdf}
\end{center}
\caption{The jet mass distribution before (left) and after (right) trimming in $Z^{\prime} \rightarrow t \bar{t}$ events,
for $m(Z^{\prime})=2$~TeV and anti-$k_T$ jets with $R=1.0$. The mean number of interactions per bunch crossing is 40 (open circles),
80 (closed circles), 140 (open squares) and 200 (closed squares). The value of the pileup noise ($\sigma$) used in the topoclustering is
optimized for each value of pileup, except in the case of $\langle\mu\rangle=40$ where the value of $\sigma$ is optimized
for $\langle\mu\rangle=30$, as in 2012 data.}
\label{fig:boost}
\end{figure}

Finally, we conclude with a statement about the increased level of activity expected as the energy of a pp collider increases. The
total inelastic cross section, $74.7\pm1.7$~mb at $8$~TeV~\cite{Antchev:2013paa} is expected to grow to $80$~mb at $13$~TeV, $90$~mb at $33$~TeV,
and $105$~mb at $100$~TeV. Inelastic events with at least one track in the central region have a central track density  ($\Delta\eta \times
\Delta \phi$) of $1.0$ at $8$~TeV and will have a central charged track density  of $1.1 \pm 0.1$ at $13$~TeV, growing to $1.33 \pm 0.14$
at $30$~TeV and  $1.8 \pm 0.4$ at $100$~TeV. The transverse energy for inelastic events deposited per unit $\Delta R^2$ in the central region of the
detector has been measured  at $\sim 0.8$~GeV at $8$~TeV, and will grow to $1.0 \pm 0.15$~GeV at $13$~TeV, $1.25 \pm 0.2$~GeV at $30$~TeV, and
$1.9 \pm 0.35$~GeV at $100$~TeV. The larger inelastic cross sections and the increased activity found in each inelastic event as the
center-of-mass energy increases will add to the difficulty for carrying out precision physics measurements. 



==> QCD/qcd-bib.tex <==
%%
%%  bibliographic items can be constructed using the LaTeX format in SPIRES:
%%    see    http://www.slac.stanford.edu/spires/hep/latex.html
%%  SPIRES will also supply the CITATION line information; please include it.
%%

%%%%%
%%%%% for alphas
%%%%%

\bibitem{Beringer:1900zz}
J. Beringer et al., Phys. Rev. D 86, 010001 (2012);
http://pdg.lbl.gov/ .

%\cite{Hikasa:1992je}
\bibitem{Hikasa:1992je} 
  K.~Hikasa {\it et al.} [Particle Data Group Collaboration],
  %``Review of particle properties. Particle Data Group,''
  Phys.\ Rev.\ D {\bf 45}, S1 (1992)
  [Erratum-ibid.\ D {\bf 46}, 5210 (1992)].
  %%CITATION = PHRVA,D45,S1;%%
  %2007 citations counted in INSPIRE as of 01 Aug 2013

\bibitem{Dissertori2013}
G.~Dissertori, 
``$\as$ at an $e^+e^-$ Z factory,'' presentation at the
Snowmass energy frontier meeting, Seattle, July 2013.

%\cite{Bethke:2012jm}
\bibitem{Bethke:2012jm} 
  S.~Bethke,
  %``World Summary of $\alpha_s$ (2012),''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 234}, 229 (2013)
  [arXiv:1210.0325 [hep-ex]].
  %%CITATION = ARXIV:1210.0325;%%
  %14 citations counted in INSPIRE as of 03 Sep 2013
  
%\cite{ALEPH:2005ab}
\bibitem{ALEPH:2005ab} 
  S.~Schael {\it et al.}  [ALEPH and DELPHI and L3 and OPAL and SLD and LEP Electroweak Working Group and SLD Electroweak Group and SLD Heavy Flavour Group Collaborations],
  %``Precision electroweak measurements on the $Z$ resonance,''
  Phys.\ Rept.\  {\bf 427}, 257 (2006)
  [hep-ex/0509008].
  %%CITATION = HEP-EX/0509008;%%
  %816 citations counted in INSPIRE as of 20 Jul 2013

%\cite{Bethke:2004uy}
\bibitem{Bethke:2004uy}
  S.~Bethke,
  %``$\alpha_s$ at Zinnowitz 2004,''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 135} (2004) 345
  [hep-ex/0407021].
  %%CITATION = HEP-EX/0407021;%%
  %107 citations counted in INSPIRE as of 06 Aug 2013

%\cite{Baikov:2008jh}
\bibitem{Baikov:2008jh} 
  P.~A.~Baikov, K.~G.~Chetyrkin and J.~H.~Kuhn,
  %``Order alpha**4(s) QCD Corrections to Z and tau Decays,''
  Phys.\ Rev.\ Lett.\  {\bf 101}, 012002 (2008)
  [arXiv:0801.1821 [hep-ph]].
  %%CITATION = ARXIV:0801.1821;%%
  %195 citations counted in INSPIRE as of 20 Jul 2013

%\cite{Baikov:2012er}
\bibitem{Baikov:2012er} 
  P.~A.~Baikov, K.~G.~Chetyrkin, J.~H.~Kuhn and J.~Rittinger,
  %``Complete ${\cal O}(\alpha_s^4)$ QCD Corrections to Hadronic $Z$-Decays,''
  Phys.\ Rev.\ Lett.\  {\bf 108}, 222003 (2012)
  [arXiv:1201.5804 [hep-ph]].
  %%CITATION = ARXIV:1201.5804;%%
  %17 citations counted in INSPIRE as of 20 Jul 2013

\bibitem{TLEP_whitepaper}
  G.~Gomez-Ceballos, M.~Klute, M.~Zanetti, P.~Lenzi, M.~Bachtis, C.~Botta, C.~Bernet and P.~Janot {\it et al.},
  ``First Look at the Physics Case of TLEP,''
  arXiv:1308.6176 [hep-ex].
  %%CITATION = ARXIV:1308.6176;%%
  %1 citations counted in INSPIRE as of 10 Sep 2013

%\cite{Flacher:2008zq}
\bibitem{Flacher:2008zq} 
  H.~Flacher, M.~Goebel, J.~Haller, A.~Hocker, K.~Monig and J.~Stelzer,
  %``Revisiting the Global Electroweak Fit of the Standard Model and Beyond with Gfitter,''
  Eur.\ Phys.\ J.\ C {\bf 60}, 543 (2009)
  [Erratum-ibid.\ C {\bf 71}, 1718 (2011)]
  [arXiv:0811.0009 [hep-ph]].
  %%CITATION = ARXIV:0811.0009;%%
  %182 citations counted in INSPIRE as of 02 Aug 2013

%\cite{Schael:2013ita}
\bibitem{Schael:2013ita} 
  S.~Schael {\it et al.}  [ALEPH and DELPHI and L3 and OPAL and LEP Electroweak Working Group Collaborations],
  %``Electroweak Measurements in Electron-Positron Collisions at W-Boson-Pair Energies at LEP,''
  arXiv:1302.3415 [hep-ex].
  %%CITATION = ARXIV:1302.3415;%%
  %8 citations counted in INSPIRE as of 20 Jul 2013



%\cite{Davier:2008sk}
\bibitem{Davier:2008sk} 
  M.~Davier, S.~Descotes-Genon, A.~Hocker, B.~Malaescu and Z.~Zhang,
  %``The Determination of alpha(s) from Tau Decays Revisited,''
  Eur.\ Phys.\ J.\ C {\bf 56}, 305 (2008)
  [arXiv:0803.0979 [hep-ph]].
  %%CITATION = ARXIV:0803.0979;%%
  %140 citations counted in INSPIRE as of 02 Aug 2013

%\cite{Pich:2013sqa}
\bibitem{Pich:2013sqa} 
  A.~Pich,
  %``Review of alpha_s determinations,''
  PoS ConfinementX {\bf }, 022 (2012)
  [arXiv:1303.2262 [hep-ph]].
  %%CITATION = ARXIV:1303.2262;%%
  %8 citations counted in INSPIRE as of 02 Aug 2013


%\cite{Altarelli:2013bpa}
\bibitem{Altarelli:2013bpa} 
  G.~Altarelli,
  %``The QCD Running Coupling and its Measurement,''
  arXiv:1303.6065 [hep-ph].
  %%CITATION = ARXIV:1303.6065;%%
  %4 citations counted in INSPIRE as of 02 Aug 2013

%%%%% Hadron colliders

%\cite{Affolder:2001hn}
\bibitem{Affolder:2001hn} CDF Collaboration,
  %T.~Affolder {\it et al.}  [CDF Collaboration],
  %``Measurement of the strong coupling constant from inclusive jet production at the Tevatron $\bar{p}p$ collider,''
  Phys.\ Rev.\ Lett.\  {\bf 88}, 042001 (2002)
  [hep-ex/0108034].
  %%CITATION = HEP-EX/0108034;%%
  %57 citations counted in INSPIRE as of 20 Jul 2013

%\cite{Abazov:2009nc}
\bibitem{Abazov:2009nc} D0 Collaboration,
  % V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  %``Determination of the strong coupling constant from the inclusive jet cross section in $p\bar{p}$ collisions at sqrt(s)=1.96 TeV,''
  Phys.\ Rev.\ D {\bf 80} (2009) 111107.
  %[arXiv:0911.2710 [hep-ex]].
  %%CITATION = ARXIV:0911.2710;%%

%\cite{Malaescu:2012ts}
\bibitem{Malaescu:2012ts}
  %B.~Malaescu and P.~Starovoitov,
  %``Evaluation of the Strong Coupling Constant alpha_s Using the ATLAS Inclusive Jet Cross-Section Data,''
  Eur.\ Phys.\ J.\ C {\bf 72} (2012) 2041.
  %[arXiv:1203.5416 [hep-ph]].
  %%CITATION = ARXIV:1203.5416;%%

%\cite{Abazov:2012lua}
\bibitem{Abazov:2012lua} D0 Collaboration,
  % V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  %``Measurement of angular correlations of jets at $\sqrt{s}=1.96$ TeV and determination of the strong coupling at high momentum transfers,''
  Phys.\ Lett.\ B {\bf 718} (2012) 56.
  %[arXiv:1207.4957 [hep-ex]].
  %%CITATION = ARXIV:1207.4957;%%

\bibitem{CMS:2013} CMS Collaboration, CMS-PAS-QCD-11-003 (2012).

%\cite{Chatrchyan:2013haa}
\bibitem{Chatrchyan:2013haa} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Determination of the top-quark pole mass and strong coupling constant from the $t\bar{t}$ production cross section in pp collisions at $\sqrt{s}$ = 7 TeV,''
  arXiv:1307.1907 [hep-ex].
  %%CITATION = ARXIV:1307.1907;%%
  %1 citations counted in INSPIRE as of 30 Jul 2013

%\cite{Ridder:2013mf}
\bibitem{Ridder:2013mf} 
  A.~G.~-D.~Ridder, T.~Gehrmann, E.~W.~N.~Glover and J.~Pires,
  %``Second order QCD corrections to jet production at hadron colliders: the all-gluon contribution,''
  Phys.\ Rev.\ Lett.\  {\bf 110}, 162003 (2013)
  [arXiv:1301.7310 [hep-ph]].
  %%CITATION = ARXIV:1301.7310;%%
  %10 citations counted in INSPIRE as of 11 Jul 2013

%%%%%%%%%%%%%%%%%%%%%%%% John's table

\bibitem{AbelleiraFernandez:2012cc}
  J.~L.~Abelleira Fernandez {\it et al.}  [LHeC Study Group],
%  ``A Large Hadron Electron Collider at CERN"
%: Report on the Physics and Design Concepts for Machine and Detector,'' 
  J.Phys.G. $\bf{39}$ (2012) 075001.

%\cite{AbelleiraFernandez:2012ty}
\bibitem{AbelleiraFernandez:2012ty}
  J.~L.~Abelleira Fernandez {\it et al.}  [LHeC Study Group],
%``On the Relation of the LHeC and the LHC'',
  arXiv:1211.5102, unpublished.

\bibitem{Bruening:2013bga}
  O.~Br\"{u}ning and M.~Klein,
  %``The Large Hadron Electron Collider,''
  Mod.\ Phys.\ Lett.\ A {\bf 28} (2013) 16,  1330011
  [arXiv:1305.2090].


%\cite{Dissertori:2009ik}
\bibitem{Dissertori:2009ik} 
  G.~Dissertori, A.~Gehrmann-De Ridder, T.~Gehrmann, E.~W.~N.~Glover, G.~Heinrich, G.~Luisoni and H.~Stenzel,
  %``Determination of the strong coupling constant using matched NNLO+NLLA predictions for hadronic event shapes in e+e- annihilations,''
  JHEP {\bf 0908}, 036 (2009)
  [arXiv:0906.3436 [hep-ph]].
  %%CITATION = ARXIV:0906.3436;%%
  %53 citations counted in INSPIRE as of 30 Jul 2013

%\cite{Dissertori:2009qa}
\bibitem{Dissertori:2009qa} 
  G.~Dissertori, A.~Gehrmann-De Ridder, T.~Gehrmann, E.~W.~N.~Glover, G.~Heinrich and H.~Stenzel,
  %``Precise determination of the strong coupling constant at NNLO in QCD from the three-jet rate in electron--positron annihilation at LEP,''
  Phys.\ Rev.\ Lett.\  {\bf 104}, 072002 (2010)
  [arXiv:0910.4283 [hep-ph]].
  %%CITATION = ARXIV:0910.4283;%%
  %46 citations counted in INSPIRE as of 30 Jul 2013



%\cite{Baak:2012kk}
\bibitem{Baak:2012kk} 
  M.~Baak, M.~Goebel, J.~Haller, A.~Hoecker, D.~Kennedy, R.~Kogler, K.~Moenig and M.~Schott {\it et al.},
  %``The Electroweak Fit of the Standard Model after the Discovery of a New Boson at the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 72}, 2205 (2012)
  [arXiv:1209.2716 [hep-ph]].
  %%CITATION = ARXIV:1209.2716;%%
  %82 citations counted in INSPIRE as of 30 Jul 2013

%\cite{Gao:2013xoa}
\bibitem{Gao:2013xoa} 
  J.~Gao, M.~Guzzi, J.~Huston, H.~-L.~Lai, Z.~Li, P.~Nadolsky, J.~Pumplin and D.~Stump {\it et al.},
  %``The CT10 NNLO Global Analysis of QCD,''
  arXiv:1302.6246 [hep-ph].
  %%CITATION = ARXIV:1302.6246;%%
  %18 citations counted in INSPIRE as of 08 Jul 2013


%\cite{Alekhin:2012ig}
\bibitem{Alekhin:2012ig} 
  S.~Alekhin, J.~Blumlein and S.~Moch,
  %``Parton Distribution Functions and Benchmark Cross Sections at NNLO,''
  Phys.\ Rev.\ D {\bf 86}, 054009 (2012)
  [arXiv:1202.2281 [hep-ph]].
  %%CITATION = ARXIV:1202.2281;%%
  %80 citations counted in INSPIRE as of 08 Jul 2013


%\cite{Ball:2011us}
\bibitem{Ball:2011us} 
  R.~D.~Ball, V.~Bertone, L.~Del Debbio, S.~Forte, A.~Guffanti, J.~I.~Latorre, S.~Lionetti and J.~Rojo {\it et al.},
  %``Precision NNLO determination of alpha_s(M_Z) using an unbiased global parton set,''
  Phys.\ Lett.\ B {\bf 707}, 66 (2012)
  [arXiv:1110.2483 [hep-ph]].
  %%CITATION = ARXIV:1110.2483;%%
  %23 citations counted in INSPIRE as of 30 Jul 2013



%\cite{Martin:2009bu}
\bibitem{Martin:2009bu} 
  A.~D.~Martin, W.~J.~Stirling, R.~S.~Thorne and G.~Watt,
  %``Uncertainties on alpha(S) in global PDF analyses and implications for predicted hadronic cross sections,''
  Eur.\ Phys.\ J.\ C {\bf 64}, 653 (2009)
  [arXiv:0905.3531 [hep-ph]].
  %%CITATION = ARXIV:0905.3531;%%
  %221 citations counted in INSPIRE as of 30 Jul 2013


%\cite{Czakon:2013goa}
\bibitem{Czakon:2013goa} 
  M.~Czakon, P.~Fiedler and A.~Mitov,
  %``The total top quark pair production cross-section at hadron colliders through O(alpha_S^4),''
  arXiv:1303.6254 [hep-ph].
  %%CITATION = ARXIV:1303.6254;%%
  %18 citations counted in INSPIRE as of 11 Jul 2013


%\cite{McNeile:2010ji}
\bibitem{McNeile:2010ji} 
  C.~McNeile, C.~T.~H.~Davies, E.~Follana, K.~Hornbostel and G.~P.~Lepage,
  %``High-Precision c and b Masses, and QCD Coupling from Current-Current Correlators in Lattice and Continuum QCD,''
  Phys.\ Rev.\ D {\bf 82}, 034512 (2010)
  [arXiv:1004.4285 [hep-lat]].
  %%CITATION = ARXIV:1004.4285;%%
  %104 citations counted in INSPIRE as of 30 Jul 2013

%\cite{Shintani:2010ph}
\bibitem{Shintani:2010ph} 
  E.~Shintani, S.~Aoki, H.~Fukaya, S.~Hashimoto, T.~Kaneko, T.~Onogi and N.~Yamada,
  %``Strong coupling constant from vacuum polarization functions in three-flavor lattice QCD with dynamical overlap fermions,''
  Phys.\ Rev.\ D {\bf 82}, 074505 (2010)
  [arXiv:1002.0371 [hep-lat]].
  %%CITATION = ARXIV:1002.0371;%%
  %21 citations counted in INSPIRE as of 30 Jul 2013

%\cite{Maltman:2008bx}
\bibitem{Maltman:2008bx} 
  K.~Maltman, D.~Leinweber, P.~Moran and A.~Sternbeck,
  %``The Realistic Lattice Determination of alpha(s)(M(Z)) Revisited,''
  Phys.\ Rev.\ D {\bf 78}, 114504 (2008)
  [arXiv:0807.2020 [hep-lat]].
  %%CITATION = ARXIV:0807.2020;%%
  %30 citations counted in INSPIRE as of 30 Jul 2013

\bibitem{Mackenzie2013}
P.~Mackenzie {\it et al.}, 
``$m_c$, $m_b$, and $\as$: Lattice status and prospects''
Snowmass Meeting, July--August 2013.


%\cite{Denner:2011mq}
\bibitem{Denner:2011mq} 
  A.~Denner, S.~Heinemeyer, I.~Puljak, D.~Rebuzzi and M.~Spira,
  %``Standard Model Higgs-Boson Branching Ratios with Uncertainties,''
  Eur.\ Phys.\ J.\ C {\bf 71}, 1753 (2011)
  [arXiv:1107.5909 [hep-ph]].
  %%CITATION = ARXIV:1107.5909;%%
  %74 citations counted in INSPIRE as of 31 Jul 2013


%%%%%
%%%%% for Lattice
%%%%%

%% %\cite{McNeile:2010ji}
%% \bibitem{McNeile:2010ji} 
%%   C.~McNeile, C.~T.~H.~Davies, E.~Follana, K.~Hornbostel and G.~P.~Lepage,
%%   %``High-Precision c and b Masses, and QCD Coupling from Current-Current Correlators in Lattice and Continuum QCD,''
%%   Phys.\ Rev.\ D {\bf 82}, 034512 (2010)
%%   [arXiv:1004.4285 [hep-lat]].
%%   %%CITATION = ARXIV:1004.4285;%%
%%   %104 citations counted in INSPIRE as of 31 Jul 2013


%\cite{Chetyrkin:2009fv}
\bibitem{Chetyrkin:2009fv} 
  K.~G.~Chetyrkin, J.~H.~Kuhn, A.~Maier, P.~Maierhofer, P.~Marquard, M.~Steinhauser and C.~Sturm,
  %``Charm and Bottom Quark Masses: An Update,''
  Phys.\ Rev.\ D {\bf 80}, 074010 (2009)
  [arXiv:0907.2110 [hep-ph]].
  %%CITATION = ARXIV:0907.2110;%%
  %112 citations counted in INSPIRE as of 31 Jul 2013


%\cite{Allison:2008xk}
\bibitem{Allison:2008xk} 
  I.~Allison {\it et al.}  [HPQCD Collaboration],
  %``High-Precision Charm-Quark Mass from Current-Current Correlators in Lattice and Continuum QCD,''
  Phys.\ Rev.\ D {\bf 78}, 054513 (2008)
  [arXiv:0805.2999 [hep-lat]].
  %%CITATION = ARXIV:0805.2999;%%
  %109 citations counted in INSPIRE as of 31 Jul 2013

%% %\cite{Shintani:2010ph}
%% \bibitem{Shintani:2010ph} 
%%   E.~Shintani, S.~Aoki, H.~Fukaya, S.~Hashimoto, T.~Kaneko, T.~Onogi and N.~Yamada,
%%   %``Strong coupling constant from vacuum polarization functions in three-flavor lattice QCD with dynamical overlap fermions,''
%%   Phys.\ Rev.\ D {\bf 82}, 074505 (2010)
%%   [arXiv:1002.0371 [hep-lat]].
%%   %%CITATION = ARXIV:1002.0371;%%
%%   %21 citations counted in INSPIRE as of 31 Jul 2013

%\cite{Aoki:2009tf}
\bibitem{Aoki:2009tf} 
  S.~Aoki {\it et al.}  [PACS-CS Collaboration],
  %``Precise determination of the strong coupling constant in N(f) = 2+1 lattice QCD with the Schrodinger functional scheme,''
  JHEP {\bf 0910}, 053 (2009)
  [arXiv:0906.3906 [hep-lat]].
  %%CITATION = ARXIV:0906.3906;%%
  %43 citations counted in INSPIRE as of 31 Jul 2013

%\cite{Blossier:2012ef}
\bibitem{Blossier:2012ef} 
  B.~Blossier, P.~.Boucaud, M.~Brinet, F.~De Soto, X.~Du, V.~Morenas, O.~Pene and K.~Petrov {\it et al.},
  %``The Strong running coupling at $\tau$ and $Z_0$ mass scales from lattice QCD,''
  Phys.\ Rev.\ Lett.\  {\bf 108}, 262002 (2012)
  [arXiv:1201.5770 [hep-ph]].
  %%CITATION = ARXIV:1201.5770;%%
  %20 citations counted in INSPIRE as of 31 Jul 2013

%%%%%
%%%%% for PDF
%%%%%

%\cite{Forte:2013wc}
\bibitem{Forte:2013wc} 
  S.~Forte and G.~Watt,
  %``Progress in the Determination of the Partonic Structure of the Proton,''
  arXiv:1301.6754 [hep-ph].
  %%CITATION = ARXIV:1301.6754;%%
  %10 citations counted in INSPIRE as of 11 Jul 2013

%\cite{DeRoeck:2011na}
\bibitem{DeRoeck:2011na} 
  A.~De Roeck and R.~S.~Thorne,
  %``Structure Functions,''
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 66}, 727 (2011)
  [arXiv:1103.0555 [hep-ph]].
  %%CITATION = ARXIV:1103.0555;%%
  %21 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Perez:2012um}
\bibitem{Perez:2012um} 
  E.~Perez and E.~Rizvi,
  %``The Quark and Gluon Structure of the Proton,''
  Rep.\ Prog.\ Phys.\  {\bf 76}, 046201 (2013)
  [arXiv:1208.1178 [hep-ex]].
  %%CITATION = ARXIV:1208.1178;%%
  %4 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Bozzi:2011ww}
\bibitem{Bozzi:2011ww} 
  G.~Bozzi, J.~Rojo and A.~Vicini,
  %``The Impact of PDF uncertainties on the measurement of the W boson mass at the Tevatron and the LHC,''
  Phys.\ Rev.\ D {\bf 83}, 113008 (2011)
  [arXiv:1104.2056 [hep-ph]].
  %%CITATION = ARXIV:1104.2056;%%
  %11 citations counted in INSPIRE as of 08 Jul 2013

%\cite{Radescu:2010zz}
\bibitem{Radescu:2010zz} 
  V.~Radescu [H1 and ZEUS Collaboration],
  %``Combination and QCD analysis of the HERA inclusive cross sections,''
  PoS ICHEP {\bf 2010}, 168 (2010).
  %%CITATION = POSCI,ICHEP2010,168;%%
  %10 citations counted in INSPIRE as of 11 Jul 2013

%\cite{CooperSarkar:2011aa}
\bibitem{CooperSarkar:2011aa} 
  A.~M.~Cooper-Sarkar [ZEUS and H1 Collaborations],
  %``PDF Fits at HERA,''
  PoS EPS {\bf -HEP2011}, 320 (2011)
  [arXiv:1112.2107 [hep-ph]].
  %%CITATION = ARXIV:1112.2107;%%
  %10 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Martin:2009iq}
\bibitem{Martin:2009iq} 
  A.~D.~Martin, W.~J.~Stirling, R.~S.~Thorne and G.~Watt,
  %``Parton distributions for the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 63}, 189 (2009)
  [arXiv:0901.0002 [hep-ph]].
  %%CITATION = ARXIV:0901.0002;%%
  %1575 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Ball:2012cx}
\bibitem{Ball:2012cx} 
  R.~D.~Ball, V.~Bertone, S.~Carrazza, C.~S.~Deans, L.~Del Debbio, S.~Forte, A.~Guffanti and N.~P.~Hartland {\it et al.},
  %``Parton distributions with LHC data,''
  Nucl.\ Phys.\ B {\bf 867}, 244 (2013)
  [arXiv:1207.1303 [hep-ph]].
  %%CITATION = ARXIV:1207.1303;%%
  %43 citations counted in INSPIRE as of 08 Jul 2013

%\cite{Ball:2012wy}
\bibitem{Ball:2012wy} 
  R.~D.~Ball, S.~Carrazza, L.~Del Debbio, S.~Forte, J.~Gao, N.~Hartland, J.~Huston and P.~Nadolsky {\it et al.},
  %``Parton Distribution Benchmarking with LHC Data,''
  JHEP {\bf 1304}, 125 (2013)
  [arXiv:1211.5142 [hep-ph]].
  %%CITATION = ARXIV:1211.5142;%%
  %18 citations counted in INSPIRE as of 08 Jul 2013

%\cite{Martin:2004dh}
\bibitem{Martin:2004dh} 
  A.~D.~Martin, R.~G.~Roberts, W.~J.~Stirling and R.~S.~Thorne,
  %``Parton distributions incorporating QED contributions,''
  Eur.\ Phys.\ J.\ C {\bf 39}, 155 (2005)
  [hep-ph/0411040].
  %%CITATION = HEP-PH/0411040;%%
  %220 citations counted in INSPIRE as of 11 Jul 2013


%\cite{Carrazza:2013bra}
\bibitem{Carrazza:2013bra} 
  S.~Carrazza,
  %``Towards the determination of the photon parton distribution function constrained by LHC data,''
  arXiv:1307.1131 [hep-ph].
  %%CITATION = ARXIV:1307.1131;%%
%\cite{Carrazza:2013wua}

\bibitem{Carrazza:2013wua} 
  S.~Carrazza,
  %``Towards an unbiased determination of parton distributions with QED corrections,''
  arXiv:1305.4179 [hep-ph].
  %%CITATION = ARXIV:1305.4179;%%
  %1 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Ball:2013hta}
\bibitem{Ball:2013hta} 
  R.~D.~Ball {\it et al.}  [The NNPDF Collaboration],
  %``Parton distributions with QED corrections,''
  arXiv:1308.0598 [hep-ph].
  %%CITATION = ARXIV:1308.0598;%%

%\cite{Bierweiler:2012kw}
\bibitem{Bierweiler:2012kw} 
  A.~Bierweiler, T.~Kasprzik, H.~Kuhn and S.~Uccirati,
  %``Electroweak corrections to W-boson pair production at the LHC,''
  JHEP {\bf 1211}, 093 (2012)
  [arXiv:1208.3147 [hep-ph]].
  %%CITATION = ARXIV:1208.3147;%%
  %3 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Baglio:2013toa}
\bibitem{Baglio:2013toa} 
  J.~Baglio, L.~D.~Ninh and M.~M.~Weber,
  %``Massive gauge boson pair production at the LHC: a next-to-leading order story,''
  arXiv:1307.4331 [hep-ph].
  %%CITATION = ARXIV:1307.4331;%%
  %2 citations counted in INSPIRE as of 21 Aug 2013



%\cite{Aad:2011fc}
\bibitem{Aad:2011fc} 
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Measurement of inclusive jet and dijet production in $pp$ collisions at $\sqrt{s}=7$ TeV using the ATLAS detector,''
  Phys.\ Rev.\ D {\bf 86}, 014022 (2012)
  [arXiv:1112.6297 [hep-ex]].
  %%CITATION = ARXIV:1112.6297;%%
  %81 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Chatrchyan:2012bja}
\bibitem{Chatrchyan:2012bja} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Measurements of differential jet cross sections in proton-proton collisions at $\sqrt{s}=7$ TeV with the CMS detector,''
  Phys.\ Rev.\ D {\bf 87}, 112002 (2013)
  [arXiv:1212.6660 [hep-ex]].
  %%CITATION = ARXIV:1212.6660;%%
  %15 citations counted in INSPIRE as of 11 Jul 2013


%\cite{Aad:2013lpa}
\bibitem{Aad:2013lpa} 
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Measurement of the inclusive jet cross section in pp collisions at $\sqrt{s}$=2.76 TeV and comparison to the inclusive jet cross section at $\sqrt{s}$=7 TeV using the ATLAS detector,''
  arXiv:1304.4739 [hep-ex].
  %%CITATION = ARXIV:1304.4739;%%
  %2 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Mangano:2012mh}
\bibitem{Mangano:2012mh} 
  M.~L.~Mangano and J.~Rojo,
  %``Cross Section Ratios between different CM energies at the LHC: opportunities for precision measurements and BSM sensitivity,''
  JHEP {\bf 1208}, 010 (2012)
  [arXiv:1206.3557 [hep-ph]].
  %%CITATION = ARXIV:1206.3557;%%
  %14 citations counted in INSPIRE as of 11 Jul 2013


\bibitem{Melnikov:2006kv} 
  K.~Melnikov and F.~Petriello,
  %``Electroweak gauge boson production at hadron colliders through O(alpha(s)**2),''
  Phys.\ Rev.\ D {\bf 74}, 114017 (2006)
  [hep-ph/0609070].
  %%CITATION = HEP-PH/0609070;%%
  
  \bibitem{Gavin:2010az} 
  R.~Gavin, Y.~Li, F.~Petriello and S.~Quackenbush,
  %``FEWZ 2.0: A code for hadronic Z production at next-to-next-to-leading order,''
  Comput.\ Phys.\ Commun.\  {\bf 182}, 2388 (2011)
  [arXiv:1011.3540 [hep-ph]].
  %%CITATION = ARXIV:1011.3540;%%


\bibitem{Catani:2009sm} 
  S.~Catani, L.~Cieri, G.~Ferrera, D.~de Florian and M.~Grazzini,
  %``Vector boson production at hadron colliders: A Fully exclusive QCD calculation at NNLO,''
  Phys.\ Rev.\ Lett.\  {\bf 103}, 082001 (2009)
  [arXiv:0903.2120 [hep-ph]].
  %%CITATION = ARXIV:0903.2120;%%

\bibitem{Li:2012wna} 
  Y.~Li and F.~Petriello,
  %``Combining QCD and electroweak corrections to dilepton production in FEWZ,''
  Phys.\ Rev.\ D {\bf 86}, 094034 (2012)
  [arXiv:1208.5967 [hep-ph]].
  %%CITATION = ARXIV:1208.5967;%%


\bibitem{Bernaciak:2012hj} 
  C.~Bernaciak and D.~Wackeroth,
  %``Combining NLO QCD and Electroweak Radiative Corrections to W boson Production at Hadron Colliders in the POWHEG Framework,''
  Phys.\ Rev.\ D {\bf 85}, 093003 (2012)
  [arXiv:1201.4804 [hep-ph]].
  %%CITATION = ARXIV:1201.4804;%%

\bibitem{Barze':2013yca} 
  L.~Barze', G.~Montagna, P.~Nason, O.~Nicrosini, F.~Piccinini and A.~Vicini,
  %``Neutral current Drell-Yan with combined QCD and electroweak corrections in the POWHEG BOX,''
  Eur.\ Phys.\ J.\ C {\bf 73}, 2474 (2013)
  [arXiv:1302.4606 [hep-ph]].
  %%CITATION = ARXIV:1302.4606;%%

%%
%% Referred in alphas sec
%%
%% %\cite{Ridder:2013mf}
%% \bibitem{Ridder:2013mf} 
%%   A.~G.~-D.~Ridder, T.~Gehrmann, E.~W.~N.~Glover and J.~Pires,
%%   %``Second order QCD corrections to jet production at hadron colliders: the all-gluon contribution,''
%%   Phys.\ Rev.\ Lett.\  {\bf 110}, 162003 (2013)
%%   [arXiv:1301.7310 [hep-ph]].
%%   %%CITATION = ARXIV:1301.7310;%%
%%   %10 citations counted in INSPIRE as of 11 Jul 2013


%\cite{Czakon:2013tha}
\bibitem{Czakon:2013tha} 
  M.~Czakon, M.~L.~Mangano, A.~Mitov and J.~Rojo,
  %``Constraints on the gluon PDF from top quark pair production at hadron colliders,''
  arXiv:1303.7215 [hep-ph].
  %%CITATION = ARXIV:1303.7215;%%
  %4 citations counted in INSPIRE as of 08 Jul 2013

%%\cite{Ball:2011mu}
%\bibitem{Ball:2011mu} 
%  R.~D.~Ball, V.~Bertone, F.~Cerutti, L.~Del Debbio, S.~Forte, A.~Guffanti, J.~I.~Latorre and J.~Rojo {\it et al.},
%  %``Impact of Heavy Quark Masses on Parton Distributions and LHC Phenomenology,''
%  Nucl.\ Phys.\ B {\bf 849}, 296 (2011)
%  [arXiv:1101.1300 [hep-ph]].
%  %%CITATION = ARXIV:1101.1300;%%
%  %209 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Ball:2011uy}
%\bibitem{Ball:2011uy} 
%  R.~D.~Ball {\it et al.}  [NNPDF Collaboration],
%  %``Unbiased global determination of parton distributions and their uncertainties at NNLO and at LO,''
%  Nucl.\ Phys.\ B {\bf 855}, 153 (2012)
%  [arXiv:1107.2652 [hep-ph]].
%  %%CITATION = ARXIV:1107.2652;%%
%  %92 citations counted in INSPIRE as of 11 Jul 2013

%\cite{d'Enterria:2012yj}
\bibitem{d'Enterria:2012yj} 
  D.~d'Enterria and J.~Rojo,
  %``Quantitative constraints on the gluon distribution function in the proton from collider isolated-photon data,''
  Nucl.\ Phys.\ B {\bf 860}, 311 (2012)
  [arXiv:1202.1762 [hep-ph]].
  %%CITATION = ARXIV:1202.1762;%%
  %23 citations counted in INSPIRE as of 08 Jul 2013

%\cite{Carminati:2012mm}
\bibitem{Carminati:2012mm} 
  L.~Carminati, G.~Costa, D.~D'Enterria, I.~Koletsou, G.~Marchiori, J.~Rojo, M.~Stockton and F.~Tartarelli,
  %``Sensitivity of the LHC isolated-gamma+jet data to the parton distribution functions of the proton,''
  EPL {\bf 101}, 61002 (2013)
  [Europhys.\ Lett.\  {\bf 101}, 61002 (2013)]
  [arXiv:1212.5511 [hep-ph]].
  %%CITATION = ARXIV:1212.5511;%%
  %4 citations counted in INSPIRE as of 08 Jul 2013

%\cite{Malik:2013kba}
\bibitem{Malik:2013kba} 
  S.~A.~Malik and G.~Watt,
  %``Ratios of $W$ and $Z$ cross sections at large boson $p_T$ as a constraint on PDFs and background to new physics,''
  arXiv:1304.2424 [hep-ph].
  %%CITATION = ARXIV:1304.2424;%%
  %1 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Stirling:2012vh}
\bibitem{Stirling:2012vh} 
  W.~J.~Stirling and E.~Vryonidou,
  %``Charm production in association with an electroweak gauge boson at the LHC,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 082002 (2012)
  [arXiv:1203.6781 [hep-ph]].
  %%CITATION = ARXIV:1203.6781;%%
  %6 citations counted in INSPIRE as of 11 Jul 2013

%\cite{Aaron:2009aa}
\bibitem{Aaron:2009aa}
  F.~D.~Aaron {\it et al.}  [H1 and ZEUS Collaboration],
  %``Combined Measurement and QCD Analysis of the Inclusive e+- p Scattering Cross Sections at HERA,''
  JHEP {\bf 1001} (2010) 109
  [arXiv:0911.0884].

\bibitem{Aaron:2009kv}
 F.~D.~Aaron {\it et al.}  [H1 Collaboration],
 %``A Precision Measurement of the Inclusive ep Scattering Cross Section at HERA,''
Eur.\ Phys.\ J.\ C {\bf 64}, 561 (2009)
 [arXiv:0904.3513].

 \bibitem{James:1975dr}
 F.~James and M.~Roos,
 %``Minuit: A System for Function Minimization and Analysis of the Parameter Errors and Correlations,''
 Comput.\ Phys.\ Commun.\  {\bf 10}, 343 (1975).


\bibitem{posterEPS}
G.~Azuelos {\it et al.}, ``New Physics with the LHeC", Poster
submitted to  EPS, Stockholm, July 2013. 

%\cite{Campbell:1999ah}
\bibitem{Campbell:1999ah} 
  J.~M.~Campbell and R.~K.~Ellis,
  %``An Update on vector boson pair production at hadron colliders,''
  Phys.\ Rev.\ D {\bf 60}, 113006 (1999)
  [hep-ph/9905386].
  %%CITATION = HEP-PH/9905386;%%
  %726 citations counted in INSPIRE as of 10 Sep 2013

%\cite{Campbell:2011bn}
\bibitem{Campbell:2011bn} 
  J.~M.~Campbell, R.~K.~Ellis and C.~Williams,
  %``Vector boson pair production at the LHC,''
  JHEP {\bf 1107}, 018 (2011)
  [arXiv:1105.0020 [hep-ph]].
  %%CITATION = ARXIV:1105.0020;%%
  %217 citations counted in INSPIRE as of 17 Jul 2013

\bibitem{HiggsEuropeanStrategy2012} 
  See web-page:
  {\tt https://twiki.cern.ch/twiki/bin/view/LHCPhysics/HiggsEuropeanStrategy2012}.

%\cite{Aad:2013bjm}
\bibitem{Aad:2013bjm} 
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Measurement of hard double-parton interactions in W->lv+ 2 jet events at sqrt(s)=7 TeV with the ATLAS detector,''
  New J.\ Phys.\  {\bf 15}, 033038 (2013)
  [arXiv:1301.6872 [hep-ex]].
  %%CITATION = ARXIV:1301.6872;%%
  %12 citations counted in INSPIRE as of 17 Jul 2013

\bibitem{Andersen:2009nu} 
  J.~R.~Andersen and J.~M.~Smillie,
  %``Constructing All-Order Corrections to Multi-Jet Rates,''
  JHEP {\bf 1001}, 039 (2010)
  [arXiv:0908.2786 [hep-ph]].

\bibitem{Andersen:2011hs} 
  J.~R.~Andersen and J.~M.~Smillie,
  %``Multiple Jets at the LHC with High Energy Jets,''
  JHEP {\bf 1106}, 010 (2011)
  [arXiv:1101.5394 [hep-ph]].

%\cite{Binoth:2010ra}
\bibitem{Binoth:2010ra} 
  J.~R.~Andersen {\it et al.}  [SM and NLO Multileg Working Group Collaboration],
  %``The SM and NLO Multileg Working Group: Summary report,''
  arXiv:1003.1241 [hep-ph].
  %%CITATION = ARXIV:1003.1241;%%
  %115 citations counted in INSPIRE as of 18 Jul 2013

%\cite{Bern:2013gka}
\bibitem{Bern:2013gka} 
  Z.~Bern, L.~J.~Dixon, F.~Febres Cordero, S.~Hoeche, H.~Ita, D.~A.~Kosower, D.~Maitre and K.~J.~Ozeren,
  %``Next-to-Leading Order W + 5-Jet Production at the LHC,''
  arXiv:1304.1253 [hep-ph].
  %%CITATION = ARXIV:1304.1253;%%
  %5 citations counted in INSPIRE as of 18 Jul 2013

%%add references for LoopSim

%\cite{Rubin:2010xp}
\bibitem{Rubin:2010xp} 
  M.~Rubin, G.~P.~Salam and S.~Sapeta,
  %``Giant QCD K-factors beyond NLO,''
  JHEP {\bf 1009}, 084 (2010)
  [arXiv:1006.2144 [hep-ph]].
  %%CITATION = ARXIV:1006.2144;%%
  %43 citations counted in INSPIRE as of 15 Aug 2013

%\cite{Maitre:2013wha}
\bibitem{Maitre:2013wha} 
  D.~Ma"tre and S.~Sapeta,
  %``Simulated NNLO for high-pT observables in vector boson + jets production at the LHC,''
  arXiv:1307.2252 [hep-ph].
  %%CITATION = ARXIV:1307.2252;%%


%\cite{Campanario:2012fk}
\bibitem{Campanario:2012fk} 
  F.~Campanario and S.~Sapeta,
  %``WZ production beyond NLO for high-pT observables,''
  Phys.\ Lett.\ B {\bf 718}, 100 (2012)
  [arXiv:1209.4595 [hep-ph]].
  %%CITATION = ARXIV:1209.4595;%%
  %9 citations counted in INSPIRE as of 15 Aug 2013

%%\cite{Campanario:2013mha}
%\bibitem{Campanario:2013mha} 
%  F.~Campanario, C.~Englert, M.~Rauch, S.~Sapeta and D.~Zeppenfeld,
%  %``Di-boson and Tri-boson production at the LHC,''
%  arXiv:1307.2261 [hep-ph].
%  %%CITATION = ARXIV:1307.2261;%%

\bibitem{Frixione:2002ik} 
  S.~Frixione and B.~R.~Webber,
  %``Matching NLO QCD computations and parton shower simulations,''
  JHEP {\bf 0206}, 029 (2002)
  [hep-ph/0204244].

\bibitem{Nason:2004rx} 
  P.~Nason,
  %``A New method for combining NLO QCD with shower Monte Carlo algorithms,''
  JHEP {\bf 0411}, 040 (2004)
  [hep-ph/0409146].

\bibitem{Frixione:2007vw} 
  S.~Frixione, P.~Nason and C.~Oleari,
  %``Matching NLO QCD computations with Parton Shower simulations: the POWHEG method,''
  JHEP {\bf 0711}, 070 (2007)
  [arXiv:0709.2092 [hep-ph]].

\bibitem{Hoeche:2012ft} 
  S.~Hoeche, F.~Krauss, M.~Schonherr and F.~Siegert,
  %``W+n-jet predictions at the Large Hadron Collider at next-to-leading order matched with a parton shower,''
  Phys.\ Rev.\ Lett.\  {\bf 110}, 052001 (2013)
  [arXiv:1201.5882 [hep-ph]].

\bibitem{Alioli:2011as} 
  S.~Alioli, S.~-O.~Moch and P.~Uwer,
  %``Hadronic top-quark pair-production with one jet and parton showering,''
  JHEP {\bf 1201}, 137 (2012)
  [arXiv:1110.5251 [hep-ph]].
  
  \bibitem{Hoeche:2012yf} 
  S.~Hoeche, F.~Krauss, M.~Schonherr and F.~Siegert,
  %``QCD matrix elements + parton showers: The NLO case,''
  JHEP {\bf 1304}, 027 (2013)
  [arXiv:1207.5030 [hep-ph]].

\bibitem{Frederix:2012ps} 
  R.~Frederix and S.~Frixione,
  %``Merging meets matching in MC@NLO,''
  JHEP {\bf 1212}, 061 (2012)
  [arXiv:1209.6215 [hep-ph]].

\bibitem{Catani:2001cc} 
  S.~Catani, F.~Krauss, R.~Kuhn and B.~R.~Webber,
  %``QCD matrix elements + parton showers,''
  JHEP {\bf 0111}, 063 (2001)
  [hep-ph/0109231].

\bibitem{Lonnblad:2001iq} 
  L.~Lonnblad,
  %``Correcting the color dipole cascade model with fixed order matrix elements,''
  JHEP {\bf 0205}, 046 (2002)
  [hep-ph/0112284].

\bibitem{Mangano:2001xp} 
  M.~L.~Mangano, M.~Moretti and R.~Pittau,
  %``Multijet matrix elements and shower evolution in hadronic collisions: $W b \bar{b}$ + $n$ jets as a case study,''
  Nucl.\ Phys.\ B {\bf 632}, 343 (2002)
  [hep-ph/0108069].

\bibitem{Lavesson:2008ah} 
  N.~Lavesson and L.~Lonnblad,
  %``Extending CKKW-merging to One-Loop Matrix Elements,''
  JHEP {\bf 0812}, 070 (2008)
  [arXiv:0811.2912 [hep-ph]].

\bibitem{Lonnblad:2012ix} 
  L.~Lonnblad and S.~Prestel,
  %``Merging Multi-leg NLO Matrix Elements with Parton Showers,''
  JHEP {\bf 1303}, 166 (2013)
  [arXiv:1211.7278 [hep-ph]].

  \bibitem{Hoeche:2013mua} 
  S.~Hoeche, J.~Huang, G.~Luisoni, M.~Schoenherr and J.~Winter,
  %``Zero and one jet combined NLO analysis of the top quark forward-backward asymmetry,''
  arXiv:1306.2703 [hep-ph].

\bibitem{Nagy:2007ty} 
  Z.~Nagy and D.~E.~Soper,
  %``Parton showers with quantum interference,''
  JHEP {\bf 0709}, 114 (2007)
  [arXiv:0706.0017 [hep-ph]].

\bibitem{Hoeche:2011fd} 
  S.~Hoeche, F.~Krauss, M.~Schonherr and F.~Siegert,
  %``A critical appraisal of NLO+PS matching methods,''
  JHEP {\bf 1209}, 049 (2012)
  [arXiv:1111.1220 [hep-ph]].

\bibitem{Platzer:2012np} 
  S.~Platzer and M.~Sjodahl,
  %``Subleading $N_c$ improved Parton Showers,''
  JHEP {\bf 1207}, 042 (2012)
  [arXiv:1201.0260 [hep-ph]].

\bibitem{Alioli:2012fc} 
  S.~Alioli, C.~W.~Bauer, C.~J.~Berggren, A.~Hornig, F.~J.~Tackmann, C.~K.~Vermilion, J.~R.~Walsh and S.~Zuberi,
  %``Combining Higher-Order Resummation with Multiple NLO Calculations and Parton Showers in GENEVA,''
  arXiv:1211.7049 [hep-ph].

\bibitem{Alioli:2013vza} 
  S.~Alioli, C.~W.~Bauer, C.~Berggren, A.~Hornig, F.~J.~Tackmann, C.~K.~Vermilion, J.~R.~Walsh and S.~Zuberi,
  %``Combining Higher-Order Resummation with Multiple NLO Calculations and Parton Showers in the GENEVA Monte Carlo Framework,''
  arXiv:1305.5246 [hep-ph].

\bibitem{Andersen:2011zd} 
  J.~R.~Andersen, L.~Lonnblad and J.~M.~Smillie,
  %``A Parton Shower for High Energy Jets,''
  JHEP {\bf 1107}, 110 (2011)
  [arXiv:1104.1316 [hep-ph]].

%\cite{Kidonakis:2000gi}
\bibitem{Kidonakis:2000gi} 
  N.~Kidonakis and J.~F.~Owens,
  %``Effects of higher order threshold corrections in high E(T) jet production,''
  Phys.\ Rev.\ D {\bf 63}, 054019 (2001)
  [hep-ph/0007268].
  %%CITATION = HEP-PH/0007268;%%
  %115 citations counted in INSPIRE as of 17 Jul 2013

%\cite{Ball:2013bra}
\bibitem{Ball:2013bra} 
  R.~D.~Ball, M.~Bonvini, S.~Forte, S.~Marzani and G.~Ridolfi,
  %``Higgs production in gluon fusion beyond NNLO,''
  Nucl.\  Phys.\  B {\bf 874}, 746 (2013)
  [arXiv:1303.3590 [hep-ph]].
  %%CITATION = ARXIV:1303.3590;%%
  %10 citations counted in INSPIRE as of 17 Jul 2013

%\cite{Bonvini:2012an}
\bibitem{Bonvini:2012an} 
  M.~Bonvini, S.~Forte and G.~Ridolfi,
  %``The Threshold region for Higgs production in gluon fusion,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 102002 (2012)
  [arXiv:1204.5473 [hep-ph]].
  %%CITATION = ARXIV:1204.5473;%%
  %5 citations counted in INSPIRE as of 17 Jul 2013

\bibitem{deFlorian:2012yg}
  D.~de Florian and M.~Grazzini,
  %``Higgs production at the LHC: updated cross sections at $\sqrt{s}=8$ TeV,''
  Phys.\ Lett.\ B {\bf 718} (2012) 117
  [arXiv:1206.4133 [hep-ph]].
  %%CITATION = ARXIV:1206.4133;%%

\bibitem{Catani:2003zt}
  S.~Catani, D.~de Florian, M.~Grazzini and P.~Nason,
  %``Soft gluon resummation for Higgs boson production at hadron colliders,''
  JHEP {\bf 0307} (2003) 028
  [hep-ph/0306211].
  %%CITATION = HEP-PH/0306211;%%

%\cite{Buehler:2013fha}
\bibitem{Buehler:2013fha} 
  S.~Buehler and A.~Lazopoulos,
  %``Scale dependence and collinear subtraction terms for Higgs production in gluon fusion at N3LO,''
  arXiv:1306.2223 [hep-ph].
  %%CITATION = ARXIV:1306.2223;%%
  %3 citations counted in INSPIRE as of 17 Jul 2013

\bibitem{qcd:sforte}
Stefano Forte, private communication.

%\cite{Boughezal:2013uia}
\bibitem{Boughezal:2013uia} 
  R.~Boughezal, F.~Caola, K.~Melnikov, F.~Petriello and M.~Schulze,
  %``Higgs boson production in association with a jet at next-to-next-to-leading order in perturbative QCD,''
  JHEP {\bf 1306}, 072 (2013)
  [arXiv:1302.6216 [hep-ph]].
  %%CITATION = ARXIV:1302.6216;%%
  %8 citations counted in INSPIRE as of 17 Jul 2013

\bibitem{Anastasiou:2008tj} 
  C.~Anastasiou, R.~Boughezal and F.~Petriello,
  %``Mixed QCD-electroweak corrections to Higgs boson production in gluon fusion,''
  JHEP {\bf 0904}, 003 (2009)
  [arXiv:0811.3458 [hep-ph]].
  %%CITATION = ARXIV:0811.3458;%%

%\cite{Dittmaier}
\bibitem{Dittmaier}
S. Dittmaier, A. Huss, C. Schwinn, in preparation. 

\bibitem{cms:dijet}
CMS Collaboration, 
https://cdsweb.cern.ch/record/1547589 (2013).

%\cite{Dittmaier:2012kx}
\bibitem{Dittmaier:2012kx} 
  S.~Dittmaier, A.~Huss and C.~Speckner,
  %``Weak radiative corrections to dijet production at hadron colliders,''
  JHEP {\bf 1211}, 095 (2012)
  [arXiv:1210.0438 [hep-ph]].
  %%CITATION = ARXIV:1210.0438;%%
  %7 citations counted in INSPIRE as of 20 Jul 2013

\bibitem{atlas:Zll}
ATLAS Collaboration, 
http://cds.cern.ch/record/1525524 (2013).

\bibitem{cms:Wlnu}
CMS Collaboration, 
http://cds.cern.ch/record/1522476 (2013).

\bibitem{Becher:2013zua} 
  T.~Becher and X.~G.~iTormo,
  %``Electroweak Sudakov effects in W, Z and gamma production at large transverse momentum,''
  arXiv:1305.4202 [hep-ph].
  %%CITATION = ARXIV:1305.4202;%%
  %1 citations counted in INSPIRE as of 20 Jul 2013

\bibitem{Aad:2012en} 
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Study of jets produced in association with a $W$ boson in $pp$ collisions at $\sqrt{s}=7$ TeV with the ATLAS detector,''
  Phys.\ Rev.\ D {\bf 85}, 092002 (2012)
  [arXiv:1201.1276 [hep-ex]].
  %%CITATION = ARXIV:1201.1276;%%
 %\cite{Aad:2011qv}

\bibitem{Aad:2011qv} 
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Measurement of the production cross section for Z/gamma* in association with jets in $pp$ collisions at $\sqrt{s}=7$ TeV with the ATLAS detector,''
  Phys.\ Rev.\ D {\bf 85}, 032009 (2012)
  [arXiv:1111.2690 [hep-ex]].
  %%CITATION = ARXIV:1111.2690;%%

\bibitem{atlas:Zjets}
ATLAS Collaboration, 
http://cds.cern.ch/record/1557773 (2013).

%\cite{Chatrchyan:2011ne}
\bibitem{Chatrchyan:2011ne} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Jet Production Rates in Association with $W$ and $Z$ Bosons in $pp$ Collisions at $\sqrt{s}=7$ TeV,''
  JHEP {\bf 1201}, 010 (2012)
  [arXiv:1110.3226 [hep-ex]].
  %%CITATION = ARXIV:1110.3226;%%
  %35 citations counted in INSPIRE as of 27 Jul 2013

%\cite{Chatrchyan:2012vr}
\bibitem{Chatrchyan:2012vr} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Measurement of the Z/gamma*+b-jet cross section in pp collisions at 7 TeV,''
  JHEP {\bf 1206}, 126 (2012)
  [arXiv:1204.1643 [hep-ex]].
  %%CITATION = ARXIV:1204.1643;%%
  %17 citations counted in INSPIRE as of 27 Jul 2013

\bibitem{cms:Wbb}
CMS Collaboration, 
https://cdsweb.cern.ch/record/1537320  (2013).

%\cite{Denner:2009gj}
\bibitem{Denner:2009gj} 
  A.~Denner, S.~Dittmaier, T.~Kasprzik and A.~Muck,
  %``Electroweak corrections to W + jet hadroproduction including leptonic W-boson decays,''
  JHEP {\bf 0908}, 075 (2009)
  [arXiv:0906.1656 [hep-ph]].
  %%CITATION = ARXIV:0906.1656;%%
  %26 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Denner:2011vu}
\bibitem{Denner:2011vu} 
  A.~Denner, S.~Dittmaier, T.~Kasprzik and A.~Muck,
  %``Electroweak corrections to dilepton + jet production at hadron colliders,''
  JHEP {\bf 1106}, 069 (2011)
  [arXiv:1103.0914 [hep-ph]].
  %%CITATION = ARXIV:1103.0914;%%
  %16 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Denner:2012ts}
\bibitem{Denner:2012ts} 
  A.~Denner, S.~Dittmaier, T.~Kasprzik and A.~Mück,
  %``Electroweak corrections to monojet production at the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 73}, 2297 (2013)
  [arXiv:1211.5078 [hep-ph]].
  %%CITATION = ARXIV:1211.5078;%%
  %2 citations counted in INSPIRE as of 23 Jul 2013

\bibitem{atlas:WWllvv}
ATLAS Collaboration, 
http://cds.cern.ch/record/1562879 (2013).

\bibitem{cms:WWlnuqq}
CMS Collaboration, 
http://cds.cern.ch/record/1546778 (2013).

%\cite{Kuhn:2005az}
\bibitem{Kuhn:2005az} 
  J.~H.~Kuhn, A.~Kulesza, S.~Pozzorini and M.~Schulze,
  %``One-loop weak corrections to hadronic production of Z bosons at large transverse momenta,''
  Nucl.\ Phys.\ B {\bf 727}, 368 (2005)
  [hep-ph/0507178].
  %%CITATION = HEP-PH/0507178;%%
  %35 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Kuhn:2007cv}
\bibitem{Kuhn:2007cv} 
  J.~H.~Kuhn, A.~Kulesza, S.~Pozzorini and M.~Schulze,
  %``Electroweak corrections to hadronic production of W bosons at large transverse momenta,''
  Nucl.\ Phys.\ B {\bf 797}, 27 (2008)
  [arXiv:0708.0476 [hep-ph]].
  %%CITATION = ARXIV:0708.0476;%%
  %43 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Maina:2003is}
\bibitem{Maina:2003is} 
  E.~Maina, S.~Moretti, M.~R.~Nolten and D.~A.~Ross,
  %``One loop weak corrections to the b anti-b cross-section at TeV energy hadron colliders,''
  Phys.\ Lett.\ B {\bf 570}, 205 (2003)
  [hep-ph/0307021].
  %%CITATION = HEP-PH/0307021;%%
  %30 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Maina:2004rb}
\bibitem{Maina:2004rb} 
  E.~Maina, S.~Moretti and D.~A.~Ross,
  %``One loop weak corrections to gamma / Z hadroproduction at finite transverse momentum,''
  Phys.\ Lett.\ B {\bf 593}, 143 (2004)
  [Erratum-ibid.\ B {\bf 614}, 216 (2005)]
  [hep-ph/0403050].
  %%CITATION = HEP-PH/0403050;%%
  %26 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Moretti:2006ea}
\bibitem{Moretti:2006ea} 
  S.~Moretti, M.~R.~Nolten and D.~A.~Ross,
  %``Weak corrections to four-parton processes,''
  Nucl.\ Phys.\ B {\bf 759}, 50 (2006)
  [hep-ph/0606201].
  %%CITATION = HEP-PH/0606201;%%
  %28 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Actis:2012qn}
\bibitem{Actis:2012qn} 
  S.~Actis, A.~Denner, L.~Hofer, A.~Scharf and S.~Uccirati,
  %``Recursive generation of one-loop amplitudes in the Standard Model,''
  JHEP {\bf 1304}, 037 (2013)
  [arXiv:1211.6316 [hep-ph]].
  %%CITATION = ARXIV:1211.6316;%%
  %1 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Ciafaloni:1998xg}
\bibitem{Ciafaloni:1998xg} 
  P.~Ciafaloni and D.~Comelli,
  %``Sudakov enhancement of electroweak corrections,''
  Phys.\ Lett.\ B {\bf 446}, 278 (1999)
  [hep-ph/9809321].
  %%CITATION = HEP-PH/9809321;%%
  %118 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Beccaria:1999fk}
\bibitem{Beccaria:1999fk} 
  M.~Beccaria, P.~Ciafaloni, D.~Comelli, F.~M.~Renard and C.~Verzegnassi,
  %``Logarithmic expansion of electroweak corrections to four-fermion processes in the TeV region,''
  Phys.\ Rev.\ D {\bf 61}, 073005 (2000)
  [hep-ph/9906319].
  %%CITATION = HEP-PH/9906319;%%
  %70 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Ciafaloni:2000df}
\bibitem{Ciafaloni:2000df} 
  M.~Ciafaloni, P.~Ciafaloni and D.~Comelli,
  %``Bloch-Nordsieck violating electroweak corrections to inclusive TeV scale hard processes,''
  Phys.\ Rev.\ Lett.\  {\bf 84}, 4810 (2000)
  [hep-ph/0001142].
  %%CITATION = HEP-PH/0001142;%%
  %81 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Ciafaloni:2000rp}
\bibitem{Ciafaloni:2000rp} 
  M.~Ciafaloni, P.~Ciafaloni and D.~Comelli,
  %``Electroweak Bloch-Nordsieck violation at the TeV scale: 'Strong' weak interactions?,''
  Nucl.\ Phys.\ B {\bf 589}, 359 (2000)
  [hep-ph/0004071].
  %%CITATION = HEP-PH/0004071;%%
  %44 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Ciafaloni:2001vt}
\bibitem{Ciafaloni:2001vt} 
  M.~Ciafaloni, P.~Ciafaloni and D.~Comelli,
  %``Bloch-Nordsieck violation in spontaneously broken Abelian theories,''
  Phys.\ Rev.\ Lett.\  {\bf 87}, 211802 (2001)
  [hep-ph/0103315].
  %%CITATION = HEP-PH/0103315;%%
  %30 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Denner:2000jv}
\bibitem{Denner:2000jv} 
  A.~Denner and S.~Pozzorini,
  %``One loop leading logarithms in electroweak radiative corrections. 1. Results,''
  Eur.\ Phys.\ J.\ C {\bf 18}, 461 (2001)
  [hep-ph/0010201].
  %%CITATION = HEP-PH/0010201;%%
  %112 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Denner:2001gw}
\bibitem{Denner:2001gw} 
  A.~Denner and S.~Pozzorini,
  %``One loop leading logarithms in electroweak radiative corrections. 2. Factorization of collinear singularities,''
  Eur.\ Phys.\ J.\ C {\bf 21}, 63 (2001)
  [hep-ph/0104127].
  %%CITATION = HEP-PH/0104127;%%
  %72 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Kuhn:2004em}
\bibitem{Kuhn:2004em} 
  J.~H.~Kuhn, A.~Kulesza, S.~Pozzorini and M.~Schulze,
  %``Logarithmic electroweak corrections to hadronic Z+1 jet production at large transverse momentum,''
  Phys.\ Lett.\ B {\bf 609}, 277 (2005)
  [hep-ph/0408308].
  %%CITATION = HEP-PH/0408308;%%
  %41 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Kuhn:2005gv}
\bibitem{Kuhn:2005gv} 
  J.~H.~Kuhn, A.~Kulesza, S.~Pozzorini and M.~Schulze,
  %``Electroweak corrections to hadronic photon production at large transverse momenta,''
  JHEP {\bf 0603}, 059 (2006)
  [hep-ph/0508253].
  %%CITATION = HEP-PH/0508253;%%
  %31 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Kuhn:2007qc}
\bibitem{Kuhn:2007qc} 
  J.~H.~Kuhn, A.~Kulesza, S.~Pozzorini and M.~Schulze,
  %``Electroweak corrections to large transverse momentum production of W bosons at the LHC,''
  Phys.\ Lett.\ B {\bf 651}, 160 (2007)
  [hep-ph/0703283 [HEP-PH]].
  %%CITATION = HEP-PH/0703283;%%
  %24 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Accomando:2006hq}
\bibitem{Accomando:2006hq} 
  E.~Accomando, A.~Denner and S.~Pozzorini,
  %``Logarithmic electroweak corrections to e+ e- ---> nu(e) anti-nu(e) W+ W-,''
  JHEP {\bf 0703}, 078 (2007)
  [hep-ph/0611289].
  %%CITATION = HEP-PH/0611289;%%
  %5 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Chiesa:2013yma}
\bibitem{Chiesa:2013yma} 
  M.~Chiesa, G.~Montagna, L.~Barze`, M.~Moretti, O.~Nicrosini, F.~Piccinini and F.~Tramontano,
  %``Electroweak Sudakov Corrections to New Physics Searches at the CERN LHC,''
  arXiv:1305.6837 [hep-ph].
  %%CITATION = ARXIV:1305.6837;%%

%\cite{Mangano:2002ea}
\bibitem{Mangano:2002ea} 
  M.~L.~Mangano, M.~Moretti, F.~Piccinini, R.~Pittau and A.~D.~Polosa,
  %``ALPGEN, a generator for hard multiparton processes in hadronic collisions,''
  JHEP {\bf 0307}, 001 (2003)
  [hep-ph/0206293].
  %%CITATION = HEP-PH/0206293;%%
  %1892 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Aad:2011ib}
\bibitem{Aad:2011ib} 
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Search for squarks and gluinos using final states with jets and missing transverse momentum with the ATLAS detector in $\sqrt{s}=7$ TeV proton-proton collisions,''
  Phys.\ Lett.\ B {\bf 710}, 67 (2012)
  [arXiv:1109.6572 [hep-ex]].
  %%CITATION = ARXIV:1109.6572;%%
  %266 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Collaboration:2011ida}
\bibitem{Collaboration:2011ida} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Search for New Physics with Jets and Missing Transverse Momentum in $pp$ collisions at $\sqrt{s}=7$ TeV,''
  JHEP {\bf 1108}, 155 (2011)
  [arXiv:1106.4503 [hep-ex]].
  %%CITATION = ARXIV:1106.4503;%%
  %66 citations counted in INSPIRE as of 23 Jul 2013

%\cite{Chatrchyan:2012lia}
\bibitem{Chatrchyan:2012lia} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Search for new physics in the multijet and missing transverse momentum final state in proton-proton collisions at $\sqrt{s} = 7$ TeV,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 171803 (2012)
  [arXiv:1207.1898 [hep-ex]].
  %%CITATION = ARXIV:1207.1898;%%
  %89 citations counted in INSPIRE as of 27 Jul 2013

\bibitem{Aad:2012npa} 
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Search for the Standard Model Higgs boson in the H -> WW(*) -> l nu l nu decay mode with 4.7 /fb of ATLAS data at sqrt(s) = 7 TeV,''
  Phys.\ Lett.\ B {\bf 716}, 62 (2012)
  [arXiv:1206.0756 [hep-ex]].
  %%CITATION = ARXIV:1206.0756;%%

%\cite{Chatrchyan:2012ty}
\bibitem{Chatrchyan:2012ty} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Search for the standard model Higgs boson decaying to a $W$ pair in the fully leptonic final state in $pp$ collisions at $\sqrt{s}=7$ TeV,''
  Phys.\ Lett.\ B {\bf 710}, 91 (2012)
  [arXiv:1202.1489 [hep-ex]].
  %%CITATION = ARXIV:1202.1489;%%
  %116 citations counted in INSPIRE as of 27 Jul 2013

\bibitem{Banfi:2012yh} 
  A.~Banfi, G.~P.~Salam and G.~Zanderighi,
  %``NLL+NNLO predictions for jet-veto efficiencies in Higgs-boson and Drell-Yan production,''
  JHEP {\bf 1206}, 159 (2012)
  [arXiv:1203.5773 [hep-ph]].
  %%CITATION = ARXIV:1203.5773;%%

\bibitem{Becher:2012qa} 
  T.~Becher and M.~Neubert,
  %``Factorization and NNLL Resummation for Higgs Production with a Jet Veto,''
  JHEP {\bf 1207}, 108 (2012)
  [arXiv:1205.3806 [hep-ph]].
  
  \bibitem{Tackmann:2012bt} 
  F.~J.~Tackmann, J.~R.~Walsh and S.~Zuberi,
  %``Resummation Properties of Jet Vetoes at the LHC,''
  Phys.\ Rev.\ D {\bf 86}, 053011 (2012)
  [arXiv:1206.4312 [hep-ph]].
  %%CITATION = ARXIV:1206.4312;%%
  
  \bibitem{Banfi:2012jm} 
  A.~Banfi, P.~F.~Monni, G.~P.~Salam and G.~Zanderighi,
  %``Higgs and Z-boson production with a jet veto,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 202001 (2012)
  [arXiv:1206.4998 [hep-ph]].
  %%CITATION = ARXIV:1206.4998;%%

\bibitem{Becher:2013xia} 
  T.~Becher, M.~Neubert and L.~Rothen,
  %``Factorization and N^3LL_p+NNLO Predictions for the Higgs Cross Section with a Jet Veto,''
  arXiv:1307.0025 [hep-ph].

  \bibitem{Stewart:2013faa} 
  I.~W.~Stewart, F.~J.~Tackmann, J.~R.~Walsh and S.~Zuberi,
  %``Jet p_T Resummation in Higgs Production at NNLL'+NNLO,''
  arXiv:1307.1808 [hep-ph].
  
  \bibitem{Liu:2012sz} 
  X.~Liu and F.~Petriello,
  %``Resummation of jet-veto logarithms in hadronic processes containing jets,''
  Phys.\ Rev.\ D {\bf 87}, 014018 (2013)
  [arXiv:1210.1906 [hep-ph]].
  %%CITATION = ARXIV:1210.1906;%%
  
  \bibitem{Liu:2013hba} 
  X.~Liu and F.~Petriello,
  %``Reducing theoretical uncertainties for exclusive Higgs plus one-jet production at the LHC,''
  arXiv:1303.4405 [hep-ph].
  %%CITATION = ARXIV:1303.4405;%%

\bibitem{Berger:2010xi} 
  C.~F.~Berger, C.~Marcantonini, I.~W.~Stewart, F.~J.~Tackmann and W.~J.~Waalewijn,
  %``Higgs Production with a Central Jet Veto at NNLL+NNLO,''
  JHEP {\bf 1104}, 092 (2011)
  [arXiv:1012.4480 [hep-ph]].
  %%CITATION = ARXIV:1012.4480;%%

%\cite{Ferrera:2011bk}
\bibitem{Ferrera:2011bk} 
  G.~Ferrera, M.~Grazzini and F.~Tramontano,
  %``Associated WH production at hadron colliders: a fully exclusive QCD calculation at NNLO,''
  Phys.\ Rev.\ Lett.\  {\bf 107}, 152003 (2011)
  [arXiv:1107.1164 [hep-ph]].
  %%CITATION = ARXIV:1107.1164;%%
  %55 citations counted in INSPIRE as of 17 Jul 2013  

\bibitem{Bodwin:2013nua} 
  G.~T.~Bodwin, E.~Braaten, E.~Eichten, S.~L.~Olsen, T.~K.~Pedlar and J.~Russ,
  %``Quarkonium at the Frontiers of High Energy Physics: A Snowmass White Paper,''
  arXiv:1307.7425 [hep-ph].

%\cite{Aad:2008zzm}
\bibitem{Aad:2008zzm} 
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``The ATLAS Experiment at the CERN Large Hadron Collider,''
  JINST {\bf 3}, S08003 (2008).
  %%CITATION = JINST,3,S08003;%%
  %1964 citations counted in INSPIRE as of 15 Aug 2013
  
%\cite{Cojocaru:2004jk}
\bibitem{Cojocaru:2004jk} 
  C.~Cojocaru {\it et al.}  [ATLAS Liquid Argon EMEC/HEC Collaboration],
  %``Hadronic calibration of the ATLAS liquid argon end-cap calorimeter in the pseudorapidity region 1.6 < |eta| < 1.8 in beam tests,''
  Nucl.\ Instrum.\ Meth.\ A {\bf 531}, 481 (2004)
  [physics/0407009].
  %%CITATION = PHYSICS/0407009;%%
  %54 citations counted in INSPIRE as of 15 Aug 2013
  
%\cite{Antchev:2013paa}
\bibitem{Antchev:2013paa} 
  G.~Antchev {\it et al.}  [TOTEM Collaboration],
  %``Luminosity-Independent Measurement of the Proton-Proton Total Cross Section at $\sqrt{s}=8$  TeV,''
  Phys.\ Rev.\ Lett.\  {\bf 111}, no. 1, 012001 (2013).
  %%CITATION = PRLTA,111,012001;%%
  %2 citations counted in INSPIRE as of 04 Sep 2013

%\cite{Mishra:2013una}
\bibitem{Mishra:2013una} 
  K.~Mishra, T.~Becher, L.~Barze, M.~Chiesa, S.~Dittmaier, X.~Garcia i Tormo, A.~Huss and T.~Kasprzik {\it et al.},
  %``Electroweak Corrections at High Energies,''
  arXiv:1308.1430 [hep-ph].
  %%CITATION = ARXIV:1308.1430;%%



==> QCD/tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%


==> QCD/workshopsymbols.tex <==
%%%%   Standard symbols for use in Snowmass Working Group Proceedings%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  basic formatting macros:%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\nc}{\newcommand}  

%   text mode macros

\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}
\def\etc{{\it etc}}
\def\etal{{\it et al.}}
\def\ibid{{\it ibid}.}

\def\Acknowledgements{\bigskip  \bigskip \begin{center} \begin{large}
             \bf ACKNOWLEDGEMENTS \end{large}\end{center}}


%  equation display macros

\def\beq{\begin{equation}}
\def\eeq#1{\label{#1}\end{equation}}
\def\eeqn{\end{equation}}

%%  multiple-line equations  (use \CR as the carriage return):

\newenvironment{Eqnarray}%
   {\arraycolsep 0.14em\begin{eqnarray}}{\end{eqnarray}}
\def\beqa{\begin{Eqnarray}}
\def\eeqa#1{\label{#1}\end{Eqnarray}}
\def\eeqan{\end{Eqnarray}}
\def\CR{\nonumber \\ }

%%  reference to an equation number:

\def\leqn#1{(\ref{#1})}


% math mode macros

\nc{\ra}{\rightarrow}  
\nc{\slsh}{\slash\hspace*{-0.22cm}}
\def\Re{{\cal R \mskip-4mu \lower.1ex \hbox{\it e}\,}}
\def\Im{{\cal I \mskip-5mu \lower.1ex \hbox{\it m}\,}}

\nc{\vev}[1]{ \left\langle {#1} \right\rangle }
\nc{\bra}[1]{ \langle {#1} | }
\nc{\ket}[1]{ | {#1} \rangle }
\nc{\fb}{\,{\rm fb}^{-1}}
\nc{\ev}{{\rm eV}}
\nc{\kev}{{\rm keV}}
\nc{\Mev}{{\rm MeV}}
\nc{\gev}{{\rm GeV}}
\nc{\tev}{{\rm TeV}}
\nc{\mev}{{\rm MeV}}

%%  caligraphic letters (for matrix elements, luminosity, etc.)

\def\D{{\cal D}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\O{{\cal O}}
\def\W{{\cal W}}

\def\del{\partial}
\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\def\dslash{\not{\hbox{\kern-2pt $\del$}}}
\def\pslash{\not{\hbox{\kern-2pt $p$}}}
\def\ETmiss{ \not{\hbox{\kern-4pt $E$}}_T }


%%  matrix operations and fractions:

\def\One{\ensuremath{\bf 1}\xspace}
\def\hc{\ensuremath{\mbox{\rm h.c.}}\xspace}
\def\tr{\ensuremath{\mbox{\rm tr}}\xspace}
\def\half{\ensuremath{\frac{1}{2}}\xspace}
\def\thalf{\ensuremath{\frac{3}{2}}\xspace}
\def\third{\ensuremath{\frac{1}{3}}\xspace}
\def\tthird{\ensuremath{\frac{2}{3}}\xspace}



%%  HEP terminology:

\def\Pl{{\mbox{\scriptsize Pl}}}
\def\lum{{\cal L}}
\def\eff{{\mbox{\scriptsize eff}}}
\def\CM{{\mbox{\scriptsize CM}}}
\def\BR{\mbox{\rm BR}}
\def\ee{e^+e^-}
\def\ppb{{\mbox{p\bar p}}}
\def\qqb{{\mbox{q\bar q}}}
\def\inpb{{\mbox{{\rm pb}^{-1}}}}
\def\infb{{\mbox{{\rm fb}^{-1}}}}
\def\sstw{\sin^2\theta_w}
\def\cstw{\cos^2\theta_w}
\def\mz{m_Z}
\def\gz{\Gamma_Z}
\def\mw{m_W}
\def\mt{m_t}
\def\gt{\Gamma_t}
\def\mh{m_h}
\def\gmu{G_\mu}
\def\GF{G_F}
\def\alphas{\alpha_s}
\def\msb{{\bar{\ssstyle M \kern -1pt S}}}
\def\lmsb{\Lambda_{\msb}}
\def\ELER{e^-_Le^+_R}
\def\EREL{e^-_Re^+_L}
\def\ELEL{e^-_Le^+_L}
\def\ERER{e^-_Re^+_R}
\def\eps{\epsilon}

%% supersymmetry:

\def\ch#1{\ensuremath{\widetilde\chi^+_{#1}}\xspace}
\def\chm#1{\ensuremath{\widetilde\chi^-_{#1}}\xspace}
\def\neu#1{\ensuremath{\widetilde\chi^0_{#1}}\xspace}
\def\s#1{\ensuremath{\widetilde{#1}}\xspace}

%%   experiment names

\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}








==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

